Weakly Learning to Match Experts in Online Community

In online question-and-answer (QA) websites like Quora, one central issue is to find (invite) users who are able to provide answers to a given question and at the same time would be unlikely to say "no" to the invitation. The challenge is how to trade off the matching degree between users' expertise and the question topic, and the likelihood of positive response from the invited users. In this paper, we formally formulate the problem and develop a weakly supervised factor graph (WeakFG) model to address the problem. The model explicitly captures expertise matching degree between questions and users. To model the likelihood that an invited user is willing to answer a specific question, we incorporate a set of correlations based on social identity theory into the WeakFG model. We use two different genres of datasets: QA-Expert and Paper-Reviewer, to validate the proposed model. Our experimental results show that the proposed model can significantly outperform (+1.5-10.7% by MAP) the state-of-the-art algorithms for matching users (experts) with community questions. We have also developed an online system to further demonstrate the advantages of the proposed method.

==> problem.tex <==
\section{Problem Definition}
\label{sec:problem} 



Given a query (i.e., question/paper) $q$, our goal is to find 
%the reviewer recommendation problem is given a submitted paper, to find those 
%researchers 
experts with sufficient knowledge 
who are willing to answer the question or review the paper. 
%We believe whether a researcher is proper to reviewe the paper, depends on the attributes of the researcher, the paper, the relevance between them, and also the correlation between different researchers. So w
We consider a set of $N$ candidate experts $E=\{e_1, \cdots, e_N\}$. Each expert $e_i$ corresponds to $k_i$ documents $D_i=\{d_{i,1},\cdots,d_{i,k_i}\}$, which could be questions the expert has answered, or papers the expert has published. The problem of matching questions/papers with experts can be formalized as a ranking problem. Specifically, we aim to design a ranking function which outputs $S=\{s_1,\cdots, s_N\}$, representing the ranking scores of the experts. 
Conventionally, $s_i$ is simply defined as the expertise matching score between $q$ and the expert $e_i$. In our work, we further predict whether the experts will agree to respond. More precisely, we learn a predictive function $f: (q, e_i)\rightarrow y_i$, where $y_i\in\{0,1\}$ indicates whether expert $e_i$ will respond query $q$. Finally, we rank the experts according to the probability of agreeing to respond, i.e., we define $s_i=P(y_i=1)$.



\hide{
We consider a  social network $G=(V, E)$, where $V$ is a set of $|V|=N$ experts and $E\subseteq V\times V$ is a set of relationships between experts. There can be various kinds of  relationships in different social networks. For example, in an academic social network, the relationships can be collaborations, %same-affiliation, and same-nationality; 
while in a Quora-like network, the relationships include friendship, reply, and co-reply.  Let $\mathbf{a}_i$ denote expert $e_i$'s attributes, which could be one's interests, the questions she/he has replied,  or simply the number of the posts. $A=\{\mathbf{a}_1,\cdots,\mathbf{a}_N\}$ denotes the attributes of all experts. 
Given these definitions, we  define our problem of finding proper experts as follows.
%Precisely, we can define the following problem:

\hide{
similar research interests, 
We believe whether a researcher is proper to reviewe the paper, depends on the attributes of the researcher, the paper, the relevance between them, and also the correlation between different researchers. So w
}

%\newtheorem{problem}{Problem}
\begin{problem}
\textbf{Expertise Matching with Declination Prediction.} Let $G=(V, E, A)$ be an attribute-augmented social network. Given a particular question $q$, the goal is to design a predictive function such that we can suggest experts of high relevance to question $q$ and of low risk of declining the review invitation, i.e.,
\beq{f:(G,q)\to Y}
\noindent where $Y=\{y_1,\cdots,y_N\}$ represents the prediction results for all experts in the network $G$ and $y_i\in\{0,1\}$ is a binary score indicating whether expert $e_i\in V$ has a high risk of declining the invitation.
\end{problem}
%\jz{so $y_k$ is to indicate declination, not relevance. or both?}

The predictive function $f$ takes the network $G$ as input, which means that we should consider the network information in designing the predictive function. 
Additionally, another technical challenge is how to consider both expertise matching and the potential of declination.
%We also demonstrate that the network information is very useful and can help improve the prediction accuracy.
}

